From Layers to States: A State Space Model Perspective to Deep Neural Network Layer Dynamics

The depth of neural networks is a critical factor for their capability, with deeper models often demonstrating superior performance. Motivated by this, significant efforts have been made to enhance layer aggregation - reusing information from previous layers to better extract features at the current layer, to improve the representational power of deep neural networks. However, previous works have primarily addressed this problem from a discrete-state perspective which is not suitable as the number of network layers grows. This paper novelly treats the outputs from layers as states of a continuous process and considers leveraging the state space model (SSM) to design the aggregation of layers in very deep neural networks. Moreover, inspired by its advancements in modeling long sequences, the Selective State Space Models (S6) is employed to design a new module called Selective State Space Model Layer Aggregation (S6LA). This module aims to combine traditional CNN or transformer architectures within a sequential framework, enhancing the representational capabilities of state-of-the-art vision networks. Extensive experiments show that S6LA delivers substantial improvements in both image classification and detection tasks, highlighting the potential of integrating SSMs with contemporary deep learning techniques.

==> sections/1-abstract.tex <==
\begin{abstract}

%两种思路：
%（1）从state space model这个数学模型出来，可以把network描述成一个SSM，network layer之间的interaction正好和SSM的hidden state更新相似；
% Pros: 更有开创性；Cons:但是是提出一个新问题，容易被challenge；
%（2）从layer interaction出发，指出现有的high-performance model通常具有deep layer sequence，很适合通过SSM来解决这个long sequence modeling的问题；
% Pros：是基于现有的工作，比较好写；Cons: contribution显得小一些，是基于以前工作的A+B


  Recently, state space models have gained traction across various fields, particularly in long-sequence modeling tasks. 
  %
  While most contemporary studies leverage state space models as standalone backbones, there is a notable gap in research that explores the integration of state space models with neural network architecture design.
  % While many contemporary studies leverage state space models as standalone backbones, there is a notable gap in research that explores the integration of state space models with traditional convolutional neural networks (CNNs) and transformers. 
  %
  To address this gap, our paper introduces a novel \textit{State-Space-Interaction Layer} (SSIL) model.
  %
  This innovative approach utilizes conventional transformers or CNNs as the foundational architecture while aggregating the outputs from each layer. 
  %
  The aggregated output is then fed into a state space model, generating a new sequence that enriches the model's understanding and representation of the data. 
  %
  We applied our SSAL model to both classification and detection tasks within the realm of computer vision. 
  %
  Extensive experiments demonstrated that our model not only surpassed standard models but also outperformed several existing interaction layer fusion techniques on benchmark datasets. 
  %
  This advancement highlights the potential of combining state space models with established neural network architectures, paving the way for more effective and efficient solutions in CV classification and detection tasks. 
\end{abstract}

==> sections/2-introduction.tex <==
\section{Introduction}
\label{Introduction}

Until now various statistical models have gained traction in the machine learning domain, each offering unique advantages for specific tasks. For instance, Hidden Markov Models (HMM) are frequently employed in reinforcement learning tasks, where they effectively model sequential data and capture temporal dependencies \citep{sloin2007support, dethlefs2011hierarchical}. Bayesian Networks serve as powerful tools for inference and decision support, allowing for the representation of complex relationships among variables \citep{friedman1997bayesian,chen2012good}. Additionally, Gaussian Mixture Models (GMM) excel at processing complex data distributions, making them suitable for clustering and density estimation \citep{reynolds2009gaussian,viroli2019deep}. Generative Adversarial Networks (GANs) \cite{goodfellow2020generative} and Markov chains for diffusion models \citep{sohldickstein2015deepunsupervisedlearningusing,ho2020denoisingdiffusionprobabilisticmodels} have also revolutionized image generation tasks, enabling the creation of highly realistic images through adversarial training. And now the State Space Model (SSM), as a traditional framework, is widely utilized in computer vision (CV) \citep{gu2023mamba,liu2024vmamba} tasks. Therefore, it is only natural for us to focus our attention on this model.

%
% (1) model depth在增加，depth对performance很重要: 举例子，xx model有上百layer（画一个图：performance(y-axis) vs. depth(x-axis)）；（得写之前大家是怎么解决这个问题的，但是，他们缺乏有理论支撑的数学模型的支撑的）
% 分段
% (2) 介绍SSM，点出SSM是一个有理论支撑数学模型，同时他最适合处理long sequence modelling（会介绍到H，A，B）;
% 分段
% (3) 我们propose，Network 实际上可以建模为一个SSM，那么，very deep network的layer aggregation可以formulate成一个long sequence modeling task，为什么需要设计一个SSIL（其实是因为SSM里有H，A，B）；
% (4) 具体的module设计（具体怎么在CNN/ViT），和experimental results，总结contribution：
%   a. novel formulation of Network;
%   b. 提出SSIL；
%   c. 在CV上验证了我们的propose的有效性；
% 画图：overview;CNN;ViT.

Meanwhile, recent researches have increasingly highlighted the importance of strengthening layer interactions within deep neural networks. Studies show that enhancing these interactions can significantly improve the flow of information throughout the network \citep{he2016deep,huang2018denselyconnectedconvolutionalnetworks,zhao2021recurrence,fang2023cross}. 


As our known, it is apparently that longer layer models give the better performance in vision works since it can capture more information. Therefore, some combination of models (CNNs \citep{he2016deep,ronneberger2015unetconvolutionalnetworksbiomedical,tan2020efficientnetrethinkingmodelscaling} or transformers \citep{dosovitskiy2020image,touvron2021training,liu2021swin,wang2022pvt}) appeared and they all use the larger receptive fields to capture the global semantic features. While some papers proved that encouraging interactions between layers can enhance the network's representational power by effectively combining features at different levels of abstraction. Notable architectures have emerged that exemplify this approach. ResNet \citep{he2016deep} introduced skip connections, allowing gradients to flow more easily during training by connecting non-adjacent layers. DenseNet \citep{huang2018denselyconnectedconvolutionalnetworks} took this concept further by enabling each layer to access all preceding layers within a stage, thereby fostering a rich exchange of information. More recently, GLOM \citep{hinton2023represent} adopted an intensely interactive architecture that incorporates bottom-up, top-down, and same-level connections, aiming to represent part-whole hierarchies effectively.

Building on these foundations, smaller receptive fields effectively capture local texture features, while larger receptive fields encompass more global information. This insight into the importance of layer interactions in large models inspires us to propose a novel perspective: neural networks can be conceptualized as state space models (SSMs). By leveraging the interactions between layers, outputs from different layers can be interpreted as sequential data, which serves as input to an SSM. This integration enables the SSM to encapsulate a richer representation of the information derived from the original data. Such a framework not only enhances the network's performance across various tasks but also provides a cohesive perspective that bridges traditional statistical methods with contemporary deep learning techniques. To the best of our knowledge, our work represents the first systematic investigation into cross-layer interaction within the context of SSMs. This approach distinguishes itself from existing methodologies by emphasizing the dynamic interplay between layers in neural networks, potentially leading to enhanced performance in various tasks. For CNNs-based models such as ResNet \cite{he2016deep}, and transformer-based model such as Deit \cite{touvron2021training}, Swin-Transformer \cite{liu2021swin} and PVT-v2 \cite{wang2022pvt}, we introduce a novel structure to integrate existing traditional models into sequential architectures. With the proposed State-Space-Interaction-Layer (SSIL), we effectively leverage the benefits of interactions in large-layer models while incorporating statistical models into vision tasks. By conceptualizing neural networks as state space models, we pave the way for new research avenues that bridge traditional statistical methods with contemporary deep learning techniques.

Our contributions contains:
% cv在最后一个contribution说就可以，只是一个验证的方式
\begin{enumerate}
    \item We propose that deep neural networks used in computer vision tasks can also be conceptualized as state space models. To our knowledge, this is the first time such a perspective has been presented. Our approach redefines how to utilize state space models to integrate different layers, advancing traditional multi-layer models.
    \item We introduce the State-Space-Interaction-Layer (SSIL), which conceptualizes neural networks as state space models (SSMs) to enhance cross-layer interactions. This framework integrates traditional CNNs, like ResNet, and transformer-based models, such as Deit and Swin Transformer, into sequential architectures, representing the first systematic investigation of such interactions within SSMs.
    \item In comparison with other state-of-the-art methods focusing on layer interactions—such as the ResNet \cite{he2016deep} architecture and transformer-based models like Deit \cite{touvron2021training}, Swin Transformer \cite{liu2021swin}, and PVT-v2 \cite{wang2022pvt}—our method demonstrates superior performance in classification, detection, and instance segmentation tasks.
\end{enumerate}


==> sections/4-1-methodology_mamba_hfq.tex <==
\section{Primarily State Space Model}

 And the detail proofs of Equation \eqref{eq:SSM_con} to \eqref{eq:SSM_dis} are shown as followings:
\begin{equation}
\label{eq:SSM_Parallel}
    \begin{aligned}
        h_0 & = 0 \\
        h_1 & = \overline{B} x_1 \\
        h_2 & = \overline{A}\overline{B}x_1+\overline{B}x_2 \\
        h_3 & = \overline{A}^2\overline{B}x_1+\overline{A}\overline{B}x_2+\overline{B}x_3 \\
        & \quad \vdots \\
        h_t & = \overline{A}^{t-1}\overline{B}x_1 + \overline{A}^{t-2}\overline{B}x_2 + \cdots + \overline{B}x_t. \\
    \end{aligned}
\end{equation}

Since the continuous formula is transformed to discrete form and it can be trained in parallel. Therefore, for the details of sequence-to-sequence transformation, it follows:
\begin{equation}
\label{eq:SSM_formula}
    h_t = \sum_{j=0}^{t-1} \overline{A}^j \overline{B} x_{t-j}.
\end{equation}
This is a feedforward form and this is mainly caused by the power $j$ of transition matrix $\overline{A}$ where $1 \leq j \leq t-1$. Therefore, it is an effort to block diagonalize $\overline{A}$ such that the Mamba form can be broken down more simply.

Now suppose that the transition matrix $\overline{A}$ has rank $R \leq d$. With loss of generality, we can assume that the nonzero eigenvalues of $\overline{A}$ are all distinct. Obviously, $\overline{A}$ has real nonzero eigenvalues and complex eigenvalues and the number are $r$ and $s$ respectively. Therefore the eigenvalues can be written as $\lambda_1,\cdots,\lambda_r,\lambda_{r+1},\lambda_{r+2s}$, where $(\lambda_{r+2k-1},\lambda_{r+2k}) = (\gamma_k e^{i\theta},\gamma_k e^{-i\theta})$ and $R=r+2s$ for $1 \leq i \leq s$ where $i$ is the imaginary unit. 

Therefore it is obvious that we can use Jordan decomposition \citep{} to rewrite the form of $\overline{A}^j$: $\overline{A}^j = \boldsymbol{T J}^j \boldsymbol{T}^{-1}$ where $\boldsymbol{T} \in \mathbb{R}^{d \times d}$ is invertible and $\boldsymbol{J} \in \mathbb{R}^{d \times d}$ is a Jordan block diagonal matrix. With this decomposition, the complex matrix can be broken down into some similar Jordan blocks with the dimension $p \times p$ matrix in $\boldsymbol{J}$ where $p=1$ or $2$. Therefore $\boldsymbol{J} = \text{diag}\{\lambda_1,\cdots,\lambda_r,\boldsymbol{C}_1,\cdots,\boldsymbol{C}_s,\boldsymbol{0}\}$, where $\boldsymbol{C}_k$ follows:

$$
\boldsymbol{C}_k=\gamma_k \cdot\left(\begin{array}{cc}
\cos (\theta_k) & \sin (\theta_k) \\
-\sin (\theta_k) & \cos (\theta_k)
\end{array}\right) \in \mathbb{R}^{2 \times 2}, \quad 1 \leq k \leq s.
$$

Then the form of formula \eqref{eq:SSM_formula} can be rewritten like this: 
\begin{equation}
    h_t = \sum_{j=0}^{t-1} \overline{A}^j \overline{B} x_{t-j}=\sum_{j=0}^{t-1} \boldsymbol{T}\boldsymbol{J}^j \boldsymbol{T}^{-1}\overline{B} x_{t-j}.
\end{equation}
Since $\boldsymbol{J}$ has a real Jordan form, $h_t$ follows:
\begin{equation}
\label{eq:SSM_Jordan}
    \begin{aligned}
        h_t & = \sum_{j=0}^{t-1} \boldsymbol{T}\boldsymbol{J}^j \boldsymbol{T}^{-1}\overline{B} x_{t-j} \\
        & = \sum_{j=1}^{t-1}\sum_{k=1}^r \lambda_k^j \boldsymbol{M}_k^R \overline{B}x_{t-j}+\sum_{j=1}^{t-1}\sum_{k=1}^s \gamma_k^j \{\cos(j\theta_k)\boldsymbol{M}_k^{C_1}+\sin(j\theta_k)\boldsymbol{M}_k^{C_2}\} \overline{B}x_{t-j}+\overline{B}x_t \\
        & = \sum_{k=1}^r h_t^R(\lambda_k) + \sum_{k=1}^s h_t^{C_1}(\gamma_k,\theta_k)+\sum_{k=1}^s h_t^{C_2}(\gamma_k,\theta_k)+ \overline{B}x_t,
    \end{aligned}
\end{equation}
where $h_t^R(\lambda_k) = \sum_{j=1}^{t-1}\boldsymbol{M}_k^R \overline{B}x_{t-j}$, $h_t^{C_1}(\gamma_k,\theta_k)=\sum_{j=1}^{t-1}\gamma_k^j \cos(j\theta_k)\boldsymbol{M}_k^{C_1}\overline{B}x_{t-j}$ and $h_t^{C_2}(\gamma_k,\theta_k)=\sum_{j=1}^{t-1}\gamma_k^j \sin(j\theta_k)\boldsymbol{M}_k^{C_2}\overline{B}x_{t-j}$. $\boldsymbol{M}_k^R,\boldsymbol{M}_k^{C_1},\boldsymbol{M}_k^{C_2}$ represent the real metrics determined jointly by $\boldsymbol{T}$ and $\boldsymbol{T}^{-1}$ and they are the functions of $\Delta A$ which can be written as $g_1(\Delta A)$ and the function $g$ is trainable. $\overline{B}$ is the combination of function $\Delta A$ and $B$ which can be written as $g_2(\Delta A) \otimes f(B)$.

Followed by Equation \ref{eq:SSM_Jordan}, the state space model has been broken down to three parts: real decomposition part, complex decomposition part and constant decomposition part.

\subsection{Mamba insert into Multi-head self attention}

Consider the input of self attention mechanism $X = (x_1,x_2,\cdots,x_T)' \in \mathbb{R}^{T \times d_{in}}$, a standard transformer contains Query, Key and Value. And the self attention mechanism is as following:
\begin{equation}
\label{eq:SA}
Attention(\boldsymbol{Q},\boldsymbol{K},\boldsymbol{V}) = \text{Softmax}(\boldsymbol{QK}')\boldsymbol{V},
\end{equation}
where $\boldsymbol{Q}$, $\boldsymbol{K}$ and $\boldsymbol{V}$ are all linear projection from input $X$. In this way, Mamba can be inserted into transformer and with the advantages of Mamba structure which can obtain the sequential properties, we combine this idea into the positional embedding used to keep sequential in transformer. Therefore it can be represented as this form:
\begin{equation}
SA(\boldsymbol{Q},\boldsymbol{K},\boldsymbol{V}) = \text{Softmax}(\boldsymbol{QK}'+\textbf{P})\boldsymbol{V},
\end{equation}
where $\textbf{P}$ is the positional embedding given by Mamba. And the form of $\textbf{P}$ is shown as two parts next:

$$
\mathbf{P}^R(\lambda)=\left(\begin{array}{ccccc}
0 & 0 & 0 & \cdots & 0 \\
f_1(\lambda) & 0 & 0 & \cdots & 0 \\
f_2(\lambda) & f_1(\lambda) & 0 & \cdots & 0 \\
\vdots & \vdots & \vdots & \ddots & \vdots \\
f_{T-1}(\lambda) & f_{T-2}(\lambda) & f_{T-3}(\lambda) & \cdots & 0
\end{array}\right)
$$
$$
\mathbf{P}^{C_k}(\gamma,\theta)=\left(\begin{array}{ccccc}
0 & 0 & 0 & \cdots & 0 \\
g^k_1(\gamma,\theta) & 0 & 0 & \cdots & 0 \\
g^k_2(\gamma,\theta) & g^k_1(\gamma,\theta) & 0 & \cdots & 0 \\
\vdots & \vdots & \vdots & \ddots & \vdots \\
g^k_{T-1}(\gamma,\theta) & g^k_{T-2}(\gamma,\theta) & g^k_{T-3}(\gamma,\theta) & \cdots & 0
\end{array}\right),
$$

where $\mathbf{P}^R(\lambda)$ is the real decomposition part, and $\mathbf{P}^{C_k}(\gamma,\theta)$ for $k\in\{1,2\}$ are the complex decomposition part. Looking back to Equation \ref{eq:SSM_Jordan}, if we want to add Mamba structure into transformer as the positional embedding, it is clear that we can treat $\boldsymbol{M}_k^F \overline{B}$ for $F \in \{R,C_1,C_2\}$ as the linear projection from $X$ to $\boldsymbol{V}$ which is $W_V$. Therefore, for the real part, $f_t(\lambda)=\lambda^t$ for $1 \leq t \leq T-1$ and for the complex part $g_1^1(\gamma,\theta)=\gamma^t \cos(t\theta)$ and $g_1^2(\gamma,\theta)=\gamma^t \sin(t\theta)$.

For the choice of real or complex part, it is surprisingly that we can find the state space model discretization can be represented into a multi-head self attention with $r+2s+1$ heads, where the query and key matrices are zero, and the relative positional embeddings are $\{\mathbf{P}^R(\lambda_k),1 \leq k \leq r\}$, $\{\mathbf{P}^{C_i}(\gamma_k,\theta_k),i \in \{1,2\},1 \leq k \leq s\}$ and an identity matrix, respectively. Therefore, we can insert different parts of decomposition into each head. $h_t^R$ provides the regular exponential decay induced by the real eigenvalues $\lambda_k$'s and $h_t^{C_i},i\in \{1,2\}$ provide the cyclical damoped cosine or sine decay induced by the pair of complex eigenvalues with $\gamma$ and $\theta$. These temporal patterns are further summarized into $\mathbf{P}^R(\lambda_k)$ and $\mathbf{P}^{C_i}(\gamma_k,\theta_k),i \in \{1,2\}$.

\textbf{Selective Scan Mechanism.} However for mamba structure, the advantage is that it can select the importance of input. For example, for simple copy task, it is easily solved by time-invariant models such as linear recurrences and global convolutions. But for selective copying task, we should give a solution based on the input which means the selective mechanism used in Mamba. Therefore for the parameters $\Delta,B$ in Equation \ref{eq:SSM_dis}, they both depend on input $X$ which always a linear projection from $X$ to $\Delta$ and $B$. In our time series forecasting task, it is clear that the time interval is certain. So compared with other natural language process tasks, the time interval is uncertain and it is need to depend on the input. So consider the Equation \eqref{eq:SSM_dis}, $\overline{A}$ is the transition matrix which not depends on the input so we can use the Jordan decomposition to transform this into constant calculation. And for $\overline{B}$, it depends on $\Delta,A,B$ where $B$ depends on $X$ which means we can add the selective mechanism in the value projection. Compared with vanilla transformer, for the multi-head self attention, $\boldsymbol{V} = W_V X$ for $W_V \in \mathbb{R}^{d_{in} \times d}$, we transform linear projection to the selective linear projection which means replace $W_V$ from a matrix to $W_V = W_W X$ for $W_W \in \mathbb{R}^{d \times d}$ which depends on the input $X$.

\section{Combine Mamba and self attention}

For vanilla transformer models, in the self attention mechanism, it lacks of the significant sample efficiency in modeling the sequential patterns. Therefore we add the Mamba patterns into self attention to capture the recurrent parts. Also the state space model discretization can be represented into a multi-head self attention (MHSF) where the query and key are zero for a standard MHSF. These motivate us to combine the strengths of Mamba idea with MHSF:
\begin{equation}
\label{eq:MHSF}
    \text{MambaSA}(X)=\{[1-\sigma(\mu)]\text{softmax}(\boldsymbol{QK}')+\sigma(\mu)\textbf{P}\}\boldsymbol{V},
\end{equation}
where $\textbf{P}$ is a regular or cyclical part, and $\sigma(\mu)$ is the gate-control structure used to control the probability of positional embedding given by Mamba.

Also note that $\textbf{P}$ are all lower triangular matrices, which correspond to unidirectional Mamba. Therefore, from the idea of VMamba \citep{liu2024vmamba}, for a figure, this paper gives a scan approach which need to scan from top-left, bottom-right, top-right and bottom-left. While for time series dataset, it is only need two scan merge on the sequential data. Followed by \citet{huang2022encoding} and \citet{liu2024vmamba}, we propose the bidirectional Mamba scan mechanism and we define the double scan version of $\textbf{P}$ as $\textbf{P}_{bi}$ which is $\textbf{P}^R_{bi}(\lambda)=\textbf{P}^R(\lambda)+[\textbf{P}^R(\lambda)]'$ and $\textbf{P}^{C_i}_{bi}(\gamma,\theta)=\textbf{P}^{C_i}(\gamma,\theta)+[\textbf{P}^{C_i}(\gamma,\theta)]'$ for regular and cyclical part. Also in order to limit the explosive of parameters, we give the limitation of $|\lambda| \leq 1$ and $|\gamma| \leq 1$. Therefore follows \citet{huang2022encoding}, they further bound these two parameters by transformation with hyperbolic tangent function (tanh) activation function which means $\lambda = \text{tanh}(\phi)$ and $\gamma = \text{tanh}(\psi)$. Therefore, the notations become $\textbf{P}_{bi}^R(\phi)$ and $\textbf{P}_{bi}^R(\psi,\theta)$.

On one hand, comparing with the baseline Transformer, the inclusion of REMs
will lead to a significant improvement of sample efficiency in modeling the recurrent patterns (at least it will perform similar with baseline since $\sigma(\mu) \rightarrow 0$), and hence a higher accuracy in prediction can be expected from the proposed RSA. On the other hand, comparing with the traditional Mamba models, our method also considers the correlation between any two tokes with selective. And for the multihead MambaSA, the gate-control parameter $\mu$ only varies across layers, while the parameters controlling the matrix $\textbf{P}$ vary across all heads and layers.

Additionally, followed by \citet{huang2022encoding}, it is essential to use dilated variant of $\textbf{P}$. It can be further obtained by considering the block matrix formed by the first $T$ colomns and first $T$ rows of $\textbf{P} \otimes \textbf{I}_d$ where $d$ is the dilating factor. This describes the periodic of long time series, especially for the dataset used by us. Therefore our positional embeddings contain six parts, one regular $\textbf{P}^R(\phi)$, two cyclical $\textbf{P}^{C_i}(\psi,\theta)$ for $i \in \{1,2\}$, one dilated regular $\textbf{P}^R(\phi) \otimes \textbf{I}_d$ and two dilated cyclical $\textbf{P}^{C_i}(\psi,\theta) \otimes \textbf{I}_d$ for $i \in \{1,2\}$.





